Low-latency Imaging and Inference from LoRa-enabled CubeSats

Recent years have seen the rapid deployment of low-cost CubeSats in low-Earth orbit, primarily for research, education, and Earth observation. The vast majority of these CubeSats experience significant latency (several hours) from the time an image is captured to the time it is available on the ground. This is primarily due to the limited availability of dedicated satellite ground stations that tend to be bulky to deploy and expensive to rent. This paper explores using LoRa radios in the ISM band for low-latency downlink communication from CubeSats, primarily due to the availability of extensive ground LoRa infrastructure and minimal interference to terrestrial communication. However, the limited bandwidth of LoRa precludes rich satellite Earth images to be sent - instead, the CubeSats can at best send short messages (a few hundred bytes). This paper details our experience in communicating with a LoRa-enabled CubeSat launched by our team. We present Vista, a communication system that makes software modifications to LoRa encoding onboard a CubeSat and decoding on commercial LoRa ground stations to allow for satellite imagery to be communicated, as well as wide-ranging machine learning inference on these images. This is achieved through a LoRa-channel-aware image encoding that is informed by the structure of satellite images, the tasks performed on it, as well as the Doppler variation of satellite signals. A detailed evaluation of Vista through trace-driven emulation with traces from the LoRa-CubeSat launch (in 2021) shows 4.56 dB improvement in LoRa image PSNR and 1.38x improvement in land-use classification over those images.

==> text/3-motivation.tex <==
\section{Motivation Study}

\swarun{Move to Doppler section please.. A cubesat primer may go here if needed}
In this section, we present our measurement study originating from existing CubeSat deployments in 915 MHz using the LoRa modulation. We present the key challenges that these deployments typically face.

\subsection{CubeSat parameters}

\subsection{Packet Detection Problems}
One of the key observations across various passes measured by public receivers around the globe as well as our own receivers was that while a given pass should have communicated 10-15 packets, only 4-5 packets were detected. For further investigation, the CubeSat was set in the CW mode to detect its behavior across the passes. Fig.~\ref{fig:dopplervariance} shows one such sample trace over a pass.



First factor that affect packet detection is indeed the fact that across it's path overhead, the distance varies drastically causing significantly larger attenuation in the first few and the last few packets. Indeed, the difference in an ideal pass (peak at 90$^{\circ}$), can be as large as XXX dB. 

However, these detection problems for these few attenuated packets is made much worse by the fact that these same packets face the most Doppler deviation from the center frequency expected. Now one may think that as LoRa was designed to be resilient to frequency offsets, this should not affect the reception much. However, the order of offsets ($\sim$a few Hz) that the modulation was designed to be resilient for, is significantly smaller than the multiple KHz of Doppler offsets caused due to the bad combination of high center frequency and high velocity of the satellite at lower orbits. 

Indeed, at 915 MHz center frequency and 500 km orbit radius, the Doppler shift for the edge packets can be as large as 25 KHz which is almost comparable to the bandwidth of these narrowband LoRa transmissions. In fact for a 62.5 KHz bandwidth transmitter, the first packet in the extreme case could have more than a third of it's energy outside the band that the receiver is correlating at, resulting in an effective reduction in SNR of around XXX dB. Thus, the effectively detect the packets we need a new approach to receive these packets that can overcome the sum of these attenuations of around XXX dB compared to the packet at the center of a overhead pass.

\subsection{Packet Error Problems}

Now, looking more at the center packets, we see that they have the highest likelihood of getting detected. However, using simple globally use simulation models, it is easy to see that they also perceive the maximum intra-packet Doppler shift. This is due to the fact that LoRa packets are very long (~100 ms - 2s). Further, we know that LoRa modulates information in frequency shifts. This means that this variance across a packet can lead to incorrect detection of symbols across frequency, leading to bit-errors causing the CRC to fail. 

